Sequential Auctions and Externalities

In many settings agents participate in multiple different auctions that are not necessarily implemented simultaneously. Future opportunities affect strategic considerations of the players in each auction, introducing externalities. Motivated by this consideration, we study a setting of a market of buyers and sellers, where each seller holds one item, bidders have combinatorial valuations and sellers hold item auctions sequentially. Our results are qualitatively different from those of simultaneous auctions, proving that simultaneity is a crucial aspect of previous work. We prove that if sellers hold sequential first price auctions then for unit-demand bidders (matching market) every subgame perfect equilibrium achieves at least half of the optimal social welfare, while for submodular bidders or when second price auctions are used, the social welfare can be arbitrarily worse than the optimal. We also show that a first price sequential auction for buying or selling a base of a matroid is always efficient, and implements the VCG outcome. An important tool in our analysis is studying first and second price auctions with externalities (bidders have valuations for each possible winner outcome), which can be of independent interest. We show that a Pure Nash Equilibrium always exists in a first price auction with externalities.

==> external-multiunit.tex <==

\section{Sequential Multi-Item Auctions}

TODO: Should we remove this section ?/

Here we consider the case where more than one items are auctioned at a time. We
show that even when two items are auctioned at a time and bidders have
unit-demand valuations then there might not exist a $\spe$ in pure strategies. 

First we start with an example that uses gadget $\mathcal{G}_i$ and shows that
even for unit-demand bidders, it might be that for some choice of subgame
perfect equilibria of subgames, a stage game might not have a pure nash
equilibrium. Apart from $\mathcal{G}_i$ we also add two
auctions that are auctioned simultaneously in the first round and the auctions
of the gadget are auctioned sequentially after the first round. If player $b$
wins both auctions of the first round then we implement $\spe_1$ in
$\mathcal{G}_i$ otherwise $\spe_2$ is implemented. Players have no value for
the auctions of the first round. Thus in the first round the utility of player
$b$ is $2$ for winning both items and $0$ for winning some of them, while the
utility of player $c$ is $2$ for winning any of the two items. This is a
standard example of an $AND$ and an $OR$ player that has no walrasian
equilibrium and hence no First Price Item Auction Equilibrium. Hence, the first
round has no equilibrium in pure strategies.

However, it might be that by restricting the type of subgame perfect equilibria
that arise in subsequent rounds for different outcomes of the current then
there exists a pure nash equilibrium. For example in the above example if we
restrict only one type of equilibrium to arise in the gadget then we can
construct an $\spe$. However, we show that this is not true.
Particularly, in the appendix we give an example with submodular bidders where
at most $2$ items are auctioned at a time and with no $\spe$.




==> external-preliminaries.tex <==
\section{First vs Second Price Auction}\label{sec:preliminaries}

Consider a single-item auction with $n$ players with valuations $v_1,
\hdots, v_n$ in the full information setting and where the strategy space of a
player is to report some bid $b_i \in [0, \infty)$. To avoid technical
difficulties in the first price auction, suppose a player can bid, for any real
number $x$ a bid $b = x+$ which means, infinitesimally larger then $x$.
Alternatively, one could consider limits of $\epsilon$-Nash equilibria (see
\cite{Hassidim11}).

Both first and second price mechanisms allocate the item to the player
with higher bid, but they differ in the payment rule: in the first price
auction, the allocated bidder pays his bid and in the first price auction, the
allocated player pays the second highest bid. Supposing for simplicity all
players have different valuations and $v_1 > v_2 > \hdots > v_n$, it is simple
to characterize the Nash equilibria of this auction:
\begin{enumerate}
 \item \textit{First price auction}: For any number $x \in [v_2, v_1]$ there is
an equilibrium where $b_1 = x+$ and $b_i = x$ for some $i \neq 1$ and $b_j \leq
x$ for all $j \neq 1$. I.e. player $1$ always wins the item for some price
between $v_2$ and $v_1$.
 \item \textit{Second price auction}: For any number $x \in [v_2, v_1]$, player 
$1$ bids $x$ and the other players bid $b_i < x$. In this case, player $1$ gets
the item for some price between $0$ and $v_1$. The second price auction has,
nevertheless, non-efficient equilibria, where player $i > 1$ bids $b_i \geq v_1$
and all players $j \neq i$ bid $b_j \leq v_i$.
\end{enumerate}

Bidding above ones own valuation is a blatantly dominated strategy and it is a
common assumption in much of the literature that players don't overbid. This
leaves us with a single outcome for the first price auction, where $b_1 = v_2+$
and $b_2 = v_2$, and the highest valued player gets the item by the second
highest valuation. In the second price auction, the first player bidding $b_1
\in [v_2, v_1]$ and each other player bidding $b_i \in [0,v_i]$ is an
equilibrium. So, in all outcomes, the highest value player wins the item but
the price can be anything between $0$ and $v_2$. 

It is a standard argument in the second price auction the equilibrium where
each  player reports his valuation truthfully is selected, since it is a
weak-dominant strategy to report the truth - and therefore in both auctions, the
highest player would win the item for the second highest value. We explicitely
avoid type of arguments, for two
reasons: (i) Price of Anarchy bounds that don't invoke elimination of dominated
strategies are more robust; (ii) players might employ dominated strategies for
reasons external to this auction. Consider two sequential auctions of identical
items and two players that have equal value $1$ for each items and $2$ for both
items. Since the valuations are additive, one can see the auctions are
independent. However, there is an (subgame perfect) equilibrium of this game
where player $1$ bids $1$ on the first auction and if player $2$ bids zero in
the first auction, he bids $0$ in the second, otherwise he bids $1$. Player $2$
plays zero in the first auction and one in the second auction. It is easy to see
that this is a subgame perfect equilibrium and both players are playing
dominated strategies -- and nevertheless, both are better off compared to the
equilibrium where they play truthfully in both auctions.

So, we restrict ourselves to non-overbidding equilibria, but allow other types
of weakly-dominated strategies, since they can be for a player's high-level
strategy -- signaling, for example.



